A Learning Framework for Morphological Operators using Counter-Harmonic Mean

We present a novel framework for learning morphological operators using counter-harmonic mean. It combines concepts from morphology and convolutional neural networks. A thorough experimental validation analyzes basic morphological operators dilation and erosion, opening and closing, as well as the much more complex top-hat transform, for which we report a real-world application from the steel industry. Using online learning and stochastic gradient descent, our system learns both the structuring element and the composition of operators. It scales well to large datasets and online settings.

==> conclusion.tex <==
We presented a novel framework for learning morphological operators
based on the PConv convolutional layer. Our system inherently
benefits of all algorithms developed for deep-learning as it is
based on gradient. We illustrated the potential of the approach in
learning various operators ranging from simple to complex chains
such as the one of the white/black top-hats and showed its
application to the domain of steel defect detection. We showed that
having cast the problem as a neural network learning, indeed a
Morphological Convolutional Neural Network (MCNN), we can easily
create complex topology and learn advanced operators. Therefore in
future work we intend to further apply MCNN to learn in parallel
banks of morphological filters and longer filtering pipelines.

